The design, construction and performance of the MICE scintillating fibre trackers

Charged-particle tracking in the international Muon Ionisation Cooling Experiment (MICE) will be performed using two solenoidal spectrometers, each instrumented with a tracking detector based on 350 {\mu}m diameter scintillating fibres. The design and construction of the trackers is described along with the quality-assurance procedures, photon-detection system, readout electronics, reconstruction and simulation software and the data-acquisition system. Finally, the performance of the MICE tracker, determined using cosmic rays, is presented.

==> 02-Mechanical/02-02-LightGuides/02-02-LightGuides-bak.tex <==
%
%--------  Mechanical: lightguides and optical connectors
\subsection{Light-guides and optical connectors}
\label{SubSect:LightGuidesOpticalConnectors}

\subsubsection{Light-guides}
\label{SubSubSect:LightGuides}

Clear fibre lightguides are required to transport light from the
scintillating-fibre stations to the VLPC readout system.
Kuraray clear polystyrene, round, s-type, 1.05 mm$\phi$ fibre was
chosen for the light-guides.
This attenuation length of the fibre was measured to be 7.6~m and
thus, to reduce the light loss in propagation as far as possible, the
length of the clear-fibre run from station to VLPC cassette was
specified to be 4~m.
There is a 15\% loss of light at the junction between the lightguide 
and the VLPC cassette due to the step down in fibre size (the VLPC
cassettes use 935 micron fibre, but overall we achieve good contact
at the cassette.

The light-guide, a bundle of 128 clear fibres, is composed of an internal
section, which connects between the station and patch panel, and external section,
which connects between the patch panel and the VLPC cassette. 
The external light-guide is equipped with a flexible tube that shields the fibres from
room light and also protects the fibre from any damage during final assembly. 
The length of each light-guides is summarised in Table
\ref{light_guide_length}. 

The internal light-guides (Figure \ref{light_guide} top) have one 128 fibre
optical connector (1A), and 6 22 fibre optical connectors (3A). 

The connector 1A (Figure \ref{optical_connector} top-left) has 128
holes which match with those of the connector assembly 2A-E
of external light guide. 
The connector 3A (Figure \ref{optical_connector} top-right) has 22
holes configured as shown.  These connect to the station connector and
are locked by the collar 3B. 

The external light-guides (Figure \ref{light_guide} bottom) use a 128 fibre optical
connector developed by D0 at the end that interfaces to the VLPC cassette, and connector assembly 2A-E which mates to 
connector 1A of the internal waveguide. Flexible tubes F1, F2, F3, and heat-shrink tubes S1, S2,
S3, S4 form the body casing of the external waveguide.

A light-tight injection molded boot (2F) is gluded into the backside of the D0 connector and flexible tube F1 is
attached to the boot using sleeve 2G and adhesive and heat shrink tubing S1. This makes the assembly fully light tight
and adds strength. The flexible tubes F1, F2 and F3 are fixed with heat-shrink tubes S2 and S3. 


The locking ring 2B is used for securing the connector 2A to the
connector 1A of internal light-guide at patch panel. 
The optical connector D0 (Figure \ref{optical_connector} bottom-left)
has 128 holes in an arrangement of 16 x 8, which contacts with the
connector at cassette. 
The optical connector 2A (Figure \ref{optical_connector} bottom-right)
has 128 holes in an arrangement of 12 x 11, which mates with 
connector 1A of internal light-guide. 

Optical grease is applied to all optical connectors when
mating the waveguides in order to minimise light yield loss due to Frenel reflection.
 
\begin{table}
  \begin{center}
    \begin{tabular}{ccccc}
      Serial Number & Tracker & Station & Internal & External \\
      \hline
      6-10 & 1 & 5 & 1500 mm & 2500 mm \\
      16-20 & 1 & 4 & 1950 mm & 2050 mm \\
      21-25 & 1 & 3 & 2250 mm & 1750 mm \\
      26-30 & 1 & 1 & 2600 mm & 1400 mm \\
      31-35 & 1 & 2 & 2400 mm & 1600 mm \\
      36-40 & 2 & 5 & 1500 mm & 2500 mm \\
      41-45 & 2 & 4 & 1950 mm & 2050 mm \\
      46-50 & 2 & 3 & 2250 mm & 1750 mm \\
      51-55 & 2 & 2 & 2400 mm & 1600 mm \\
      56-60 & 2 & 1 & 2600 mm & 1400 mm \\
      \hline
    \end{tabular}
  \end{center}
  \caption{
    Light-guide lengths. 
    The Serial number is a tracking number marked on the connectors. 
    Tracker 1 is for the upstream spectrometer and tracker 2 for the downstream spectrometer.
    Station 5 is located nearest to the patch panel, and station 1 is
    farthest from the patch panel.
  }
  \label{light_guide_length}
\end{table}
\begin{figure}
  \begin{center}
    \includegraphics[bb=20 20 800 560, clip,width=13cm]%
    {02-Mechanical/02-02-LightGuides/Figures/light_guide.eps}
  \end{center}
  \caption{
    Drawings for internal light-guide (top), and  external light-guide
    (bottom). 
    1A, 3A, D0, 2A are optical connectors, 3B, 2B are locking
    rings.
  }
  \label{light_guide}
\end{figure}
\begin{figure}
  \begin{center}
  \includegraphics[bb=20 20 800 560, clip,width=13cm]%
    {02-Mechanical/02-02-LightGuides/Figures/optical_connector.eps}
  \end{center}
  \caption{
    Schematic view of optical connectors. 
    The connector 1A (top-left) and 3A (top-right) are for internal
    light-guide, D0 (bottom-left) and 2A (bottom-right) for external
    light-guide.
  } 
  \label{optical_connector}
\end{figure}

\subsection{Light-guide fabrication}
\label{SubSubSect:LightGuidesFabrication}

Light-guides were fabricated by G-Tech in Tsukuba,
Japan in 2006. 
The fabrication started with cutting fibres from the spool on which they came from the manufacturer (Kuraray) to a
length of about 5 m. 
A bundle of fibres is then connected to cookies at both ends in order to
perform the first transmittance measurement. 
Details of measurement are described in the next subsection.
After selecting fibres that passed good transparency test, these were cut into two, one
for the internal waveguide and the other for for the external waveguide. 
In the next step, optical connectors are attached at both end of the
bundle, then fixed with adhesive in order to perform the first polishing step.
A second transmittance measurement is then done and light-guides that past this test were
shipped to FNAL for the second and final polishing using a diamond cutter. 

\subsection{Light-guide quality assurance}
\label{SubSubSect:LightGuidesQA}

Quality assurance of the light-guides was performed at Osaka
University in Osaka, Japan in 2006. 
After a brief inspection of the fibre connections by eye, the quality of the
fibres was measured in two ways as described below. 
The first step was to check for reflected light in a fibre.
A connector surface was exposed with a strobe light, and the reflected
light was captured in a photograph taken with a digital camera (figure
\ref{reflection}).
The injected light can be reflected from a damaged point (kinks
or crack) along a fibre, which are clearly visible in the photograph of
the connector surface (see figure \ref{reflection}). 
The second step is to measure transmittance in the fibres. 
The bundle of fibres is illuminated by diffused green LED light and
transmitted light to the other ends of fibres was observed with a CCD
camera. 
The variation in light transmission in each fibre was found to be less
than 10 $\%$. 
The fraction of fibres with transmission less than 90 $\%$ (of the average) was less
than 0.7 $\%$. 
Finally, fibre mapping at both ends was checked.
All light-guides for both upstream and downstream trackers have been
produced and checked. 
\begin{figure}
  \begin{center}
    \includegraphics[bb=10 10 400 400, clip, width=6cm]%
    {02-Mechanical/02-02-LightGuides/Figures/reflection.eps}
  \end{center}
  \caption{
    Photograph of the connector surface taken by camera with flash. 
    Reflected light is seen in a fibre at the bottom.
  }
  \label{reflection}
\end{figure}
\begin{figure}
  \begin{center}
    \includegraphics[bb=100 100 750 520, clip, width=\textwidth]%
    {02-Mechanical/02-02-LightGuides/Figures/qa.eps}
  \end{center}
  \caption{
    Setup for transmittance measurement (top). 
    Diffused green LED illuminates fibres and measure the intensity
    of transmitted light by a CCD camera.  
    CCD image of transmitted light (bottom-left) is analysed and
    readout intensities of the green component in each fibre are
    checked (bottom-right). 
  }
  \label{qa_setup}
\end{figure}

\subsubsection{Optical connectors}
\label{SubSubSect:OpticalConnectors}

{\it MICE optical connectors at station }

The station optical connector to be used  is required to mate seven
350 micron scintillating fibres to one 1.05 mm clear fibre Fig. Nim9.
The connector is shown in figure \ref{Fig:StationConnector}.
The connector has gone through 2 iterations; the ones used in the
prototype stations had 18  1.05 mm holes laid out in a regular pattern
but the final connector has 22  1.05 mm holes drilled to take the
fibres. 
The connector was machined from black delrin. 
The alignment dowels are different diameters,  2mm and  2.5mm which is
to prevent any possibility of mating the connector pair in the wrong orientation. 
To ensure that the 2 halves of the connectors have no misalignment (which would
cause light loss) a set of gauges were manufactured.  
These consisted of a plate in which was set a series of dowels
accurately positioned to were the holes would be, one for each half. 
There was also an precisely drilled plate to check the accuracy of the
gauges, see figure \ref{Fig:StnConnGuageSet}.
All of the connectors when through QA using these gauges and any that
failed were discarded.
\begin{figure}
  \begin{center}
    \includegraphics[width=0.3\textwidth,bb=0 0 563 553]%
    {02-Mechanical/02-02-LightGuides/Figures/nim3.jpg}
    \includegraphics[width=0.3\textwidth,bb=0 0 210 212]%
    {02-Mechanical/02-02-LightGuides/Figures/nim4.jpg}
  \end{center}
  \caption{
    The new connector half as fitted to the station.
  }
  \label{Fig:StationConnector}
\end{figure}
\begin{figure}
  \begin{center}
    \includegraphics[width=0.8\textwidth,bb=0 0 1729 825]%
    {02-Mechanical/02-02-LightGuides/Figures/nim10.jpg}
  \end{center}
  \caption{
    The station connector gauge set.
  }
  \label{Fig:StnConnGuageSet}
\end{figure}

Figure \ref{Fig:PtchPnlConn} Shows the Optical patch panel connector
components.  
The half with the square flange is fitted to the internal wave guide.
It incorporates an O-ring to ensure a gas seal and contains 128
fibres which gives a 1 to 1 match to the VLPC cassettes. 
As in the case of the station optical connector, it is manufactured
from Delrin.
There are 6 station connectors to each patch-panel connector; although
not all of the channels in all the station connectors are used.  
\begin{figure}
  \begin{center}
    \includegraphics[width=0.8\textwidth,bb=0 0 1219 462]%
    {02-Mechanical/02-02-LightGuides/Figures/nim6.jpg}
  \end{center}
  \caption{
    Component of the patch panel connector.
  }
  \label{Fig:PtchPnlConn}
\end{figure}

The optical signal from the tracker is piped to the VLPC system via
the external fibre waveguides. 
The waveguides terminate in the D0 warm-end optical connector shown in
figure \ref{Rig:D0Conn}. 
This is an injection-moulded part also made from Delrin. 
Shown are the 128 holes for fibres, two holes (left/right) for
alignment pins and two holes (up/down) for threaded inserts. 
The typical optical transmission for this connector interface is
approximately 98%. 
Light-guide fibre of 1.05 mm diameter is used while the D0 VLPC cassette
uses fibre of 0.965 mm diameter. 
This mismatch results in a light loss of approximately 15%.
\begin{figure}
  \begin{center}
    \includegraphics[width=0.8\textwidth,bb=0 0 656 547]%
    {02-Mechanical/02-02-LightGuides/Figures/nim7.jpg}
  \end{center}
  \caption{
    D0 warm-end optical connector.
  }
  \label{Fig:D0Conn}
\end{figure}


==> MakeClean <==
#!/bin/csh -f

rm -f *.log
rm -f *.out
rm -f *.toc
rm -f *.aux
rm -f *.dvi
rm -f *.blg

find . -name '#*#' -print -exec rm '{}' \;
find . -name '*~' -print -exec rm '{}' \;

